Tunable spin and orbital Edelstein effect at (111) LaAlO$_3$/SrTiO$_3$ interface

Converting charge current into spin current is one of the main mechanisms exploited in spintronics. One prominent example is the Edelstein effect, namely the generation of a magnetization in response to an external electric field, which can be realized in systems with lack of inversion symmetry. If a system has electrons with an orbital angular momentum character, an orbital magnetization can be generated by the applied electric field giving rise to the so-called orbital Edelstein effect. Oxide heterostructures are the ideal platform for these effects due to the strong spin-orbit coupling and the lack of inversion symmetries. Beyond a gate-tunable spin Edelstein effect, we predict an orbital Edelstein effect an order of magnitude larger then the spin one at the (111) LaAlO$_3$/SrTiO$_3$ interface. We model the material as a bilayer of $t_{2g}$ orbitals using a tight-binding approach, while transport properties are obtained in the Boltzmann approach. We give an effective model at low filling which explains the non-trivial behaviour of the Edelstein response, showing that the hybridization between the electronic bands crucially impacts the Edelstein susceptibility.

==> Edelstein Effect at 111 LAO STO-4/Supplementary_old.tex <==
\clearpage
\onecolumngrid
\section{Single band model}
In a simple generalized Rashba model the spectra for low fillings can be written as a quadratic function of $\vec{k}$ and a $|\vek|$ dependent Rashba coefficient as
\begin{equation}
    \varepsilon_\sigma(|\vek|)=\frac{\beta}{2}k^2+\alpha(|\vek|)\sigma.
\end{equation}
It can be proved by explicitly make the integral~\ref{chi} that the magnetic moment is proportional to the energy splitting between the states with different spin as
\begin{equation}
    m\propto\frac{2\alpha(|\vek|)}{\beta |\vek|}.
\end{equation}
In this framework, we show in Fig.~\ref{splitting12} the energy splitting of the first two bands of the complete model as a function of $|\vek|$ and observe that a structure similar to the single doublet curves in Fig.~\ref{fig:Edelstein_chi}.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{energy_splitting_E1_E2_Del005.png}
    \caption{}
    \label{splitting12}
\end{figure}
Moreover, by inverting the relation between $\varepsilon$ and $\vek$, one can find that the peak of the red curve in Fig.~\ref{fig:Edelstein_chi}(a) is located approximately to the same fillings. However, there are some feature that are not captured by this model: the different sign of the Rashba coefficients for the second doublet has no explanation in a simple model, and the second doublet has no linear splitting and so this model is not suitable for explaining this structure. Moreover all the three curves does not saturates to zero, but to a finite constant, even changing sign with the filling.
This simple framework can explain approximately the first peak of the red curve of $\chi^S$, but diverges when more bands are filled. That even taking three different isolated bands with Rashba splitting cannot reproduce the results. 

==> Supplementary_old.tex <==
\clearpage
\onecolumngrid
\section{Single band model}
In a simple generalized Rashba model the spectra for low fillings can be written as a quadratic function of $\vec{k}$ and a $|\vek|$ dependent Rashba coefficient as
\begin{equation}
    \varepsilon_\sigma(|\vek|)=\frac{\beta}{2}k^2+\alpha(|\vek|)\sigma.
\end{equation}
It can be proved by explicitly make the integral~\ref{chi} that the magnetic moment is proportional to the energy splitting between the states with different spin as
\begin{equation}
    m\propto\frac{2\alpha(|\vek|)}{\beta |\vek|}.
\end{equation}
In this framework, we show in Fig.~\ref{splitting12} the energy splitting of the first two bands of the complete model as a function of $|\vek|$ and observe that a structure similar to the single doublet curves in Fig.~\ref{fig:Edelstein_chi}.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{energy_splitting_E1_E2_Del005.png}
    \caption{}
    \label{splitting12}
\end{figure}
Moreover, by inverting the relation between $\varepsilon$ and $\vek$, one can find that the peak of the red curve in Fig.~\ref{fig:Edelstein_chi}(a) is located approximately to the same fillings. However, there are some feature that are not captured by this model: the different sign of the Rashba coefficients for the second doublet has no explanation in a simple model, and the second doublet has no linear splitting and so this model is not suitable for explaining this structure. Moreover all the three curves does not saturates to zero, but to a finite constant, even changing sign with the filling.
This simple framework can explain approximately the first peak of the red curve of $\chi^S$, but diverges when more bands are filled. That even taking three different isolated bands with Rashba splitting cannot reproduce the results. 
